FedSAUC: A Similarity-Aware Update Control for Communication-Efficient Federated Learning in Edge Computing

Federated learning is a distributed machine learning framework to collaboratively train a global model without uploading privacy-sensitive data onto a centralized server. Usually, this framework is applied to edge devices such as smartphones, wearable devices, and Internet of Things (IoT) devices which closely collect information from users. However, these devices are mostly battery-powered. The update procedure of federated learning will constantly consume the battery power and the transmission bandwidth. In this work, we propose an update control for federated learning, FedSAUC, by considering the similarity of users' behaviors (models). At the server side, we exploit clustering algorithms to group devices with similar models. Then we select some representatives for each cluster to update information to train the model. We also implemented a testbed prototyping on edge devices for validating the performance. The experimental results show that this update control will not affect the training accuracy in the long run.

==> arxiv/macros.tex <==
% Lai-macros.tex

\newcommand\PP{\bigskip\noindent}

\newcommand\st{\textstyle \ast}
\newcommand{\dott}{\thinspace\ldotp\ldotp}
\newcommand\defeq{\stackrel{\rm def}{=}}
%\newcommand\proof{\noindent {\bf Proof}. }
%\newcommand\qed{\hfill $\Box$ \smallskip}
%\newcommand\qed{\hspace*{\fill} $\Box$ \smallskip}
\newcommand{\blist}{\begin{list}\setlength{\topsep 0pt \parsep 0pt}}
\newcommand{\elist}{\end{list}}
\newtheorem{thm}{Theorem}
\newcommand{\bthm}{\begin{thm}\begin{textit}}
\newcommand{\ethm}{\end{textit}\end{thm}}
\newtheorem{dfn}{Definition}
\newcommand{\bdfn}{\begin{dfn}\begin{textit}}
\newcommand{\edfn}{\end{textit}\end{dfn}}
\newtheorem{obn}{Observation}
\newcommand{\bobn}{\begin{obn}\begin{textit}}
\newcommand{\eobn}{\end{textit}\end{obn}}
\newtheorem{prop}{Proposition}
\newtheorem{lema}{Lemma}
\newcommand{\bdla}{\begin{lema}\begin{textit}}
\newcommand{\edla}{\end{textit}\end{lema}}
\newtheorem{pro}{Property}
\newcommand{\bpro}{\begin{pro}\begin{textit}}
\newcommand{\epro}{\end{textit}\end{pro}}
\newtheorem{cor}{Corollary}
\newtheorem{conj}{Conjecture}
\newtheorem{ex}{Example}
%\newcommand{\mod}{\mbox{mod}}
%\newcommand{\mod}{\mathop{\mathrm{mod}}}
\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}}
\newcommand{\argmax}{\mathop{\mathrm{arg\,max}}}
\newcounter{algnum1}
\newenvironment{rlist}
{\begin{list}{(\roman{algnum1})}
{\usecounter{algnum1}
 \setlength{\parsep}{0.1ex}
 \setlength{\itemsep}{0.1ex}
 \setlength{\topsep}{0.1ex}
 \setlength{\partopsep}{0.1ex}
 \setlength{\itemindent}{-15pt}
 \setlength{\parskip}{0.1ex}}}{\end{list}}

\newcounter{algnum2}
\newenvironment{alist}
{\begin{list}{(\alph{algnum2})}
{\usecounter{algnum2}
 \setlength{\parsep}{0.1ex}
 \setlength{\itemsep}{0.1ex}
 \setlength{\topsep}{0.1ex}
 \setlength{\partopsep}{0.1ex}
 \setlength{\leftmargin 0.3in}
 \setlength{\labelsep 5pt}
 \setlength{\itemindent}{-15pt}
 \setlength{\parskip}{0.1ex}}}{\end{list}}

\newcounter{algnum3}
\newenvironment{Alist}
{\begin{list}{A\alph{algnum3}.}
{\usecounter{algnum3}
 \setlength{\parsep}{0.1ex}
 \setlength{\itemsep}{0.1ex}
 \setlength{\topsep}{0.1ex}
 \setlength{\partopsep}{0.1ex}
 \setlength{\leftmargin 0.3in}
 \setlength{\labelsep 5pt}
 \setlength{\itemindent}{-15pt}
 \setlength{\parskip}{0.1ex}}}{\end{list}}

%\setlength{\textwidth}{6.1 in}
%\setlength{\textheight}{8.5in}
%\hoffset=-0.45in % 10 pts
%\voffset=-.5in
%\hoffset=-0.55in  % 11 pts

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Tseng-macros.tex

\newcommand\myqed{\hspace*{\fill} \smallskip $\rule{2mm}{2mm}$}
\newcommand\cspbox{[\hspace{-1pt}]}
\newcommand\eqdef{\stackrel{def}{=}}
\newcommand\algoskip{\parskip=0pt \parsep=0pt \itemsep=0pt}

\newcommand\lc{\lceil}
\newcommand\rc{\rceil}
\newcommand\lf{\lfloor}
\newcommand\rf{\rfloor}
\newcommand\la{\langle}
\newcommand\ra{\rangle}
\newcommand\ul{\underline}
\newcommand\ol{\overline}
\newcommand\bit{\begin{itemize}}
\newcommand\eit{\end{itemize}}
\newcommand\itcompress{\parskip=0pt \parsep=0pt \itemsep=0pt}

\newcommand{\Dfn}[1]{Definition~\ref{#1}}
\newcommand{\Eq}[1]{Eq.~(\ref{#1})}
\newcommand{\Eqs}[2]{Eqs.~(\ref{#1}) and (\ref{#2})}
\newcommand{\Ex}[1]{Example~(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Figss}[1]{Figs.~\ref{#1}}
\newcommand{\Figs}[2]{Figs.~\ref{#1} and \ref{#2}}
\newcommand{\Lema}[1]{Lemma~\ref{#1}}
\newcommand{\Pro}[1]{pro~\ref{#1}}
\newcommand{\Thm}[1]{Theorem~\ref{#1}}
\newcommand{\Cor}[1]{Corollary~\ref{#1}}
\newcommand{\Prop}[1]{Proposition~\ref{#1}}
\newcommand{\Chap}[1]{Chapter~\ref{#1}}
\newcommand{\Sec}[1]{Section~\ref{#1}}
\newcommand{\Tab}[1]{Table~\ref{#1}}
\newcommand{\Tabs}[2]{Tables~\ref{#1} and \ref{#2}}
\newcommand{\App}[1]{Appendix~\ref{#1}}

\newenvironment{dlist}
{\begin{list}{xxxxxx}{}
}
{\end{list}}


%\mathchardef\bullet=220F               % if no bullets shows, try this

\newcommand{\normalparskip}{\parskip 10pt}
\newcommand{\tideparskip}{\parskip 6pt}
\newcommand{\doublespace}{\baselineskip=22pt}
\newcommand{\tidespace}{\baselineskip=12pt}
\newcommand{\singlespace}{\baselineskip=16pt}
\newcommand{\widespace}{\baselineskip=30pt}

\newenvironment{llist}{\begin{list}{}{\setlength
        \labelwidth{.6in}\setlength\leftmargin{\labelwidth}\addtolength
        \leftmargin{\labelsep}\itemsep 5pt plus 2pt minus 2pt
        \parsep 5pt plus 2pt minus 2pt
        \def\ITEM##1{\item[{##1}]}
        \def\makelabel##1{##1\hfill}}}{\end{list}}
\newenvironment{idescription}{\begin{list}{}{\listparindent=0.25in}
        \def\Item##1{\item[{\bf ##1}]}
        }{\end{list}}

\newcommand{\ouraddress}{
        Department of Computer and Information Science\\
        The Ohio State University\\
        2036 Neil Avenue\\
        Columbus, OH 43210-1277\\
        Tel:(614)292-6552\\
        Fax:(614)292-9201\\
        E-mail: liu@cis.ohio-state.edu
}

% Define double brackets
%
\newcommand{\ldb}{[\hspace{-2pt}[}      % left double bracket
\newcommand{\rdb}{]\hspace{-2pt}]}      % right double bracket
\newcommand{\bldb}{{\bf\ldb}}           % bold face left double bracket
\newcommand{\brdb}{{\bf\rdb}}           % bold face right double bracket
\newcommand{\db}[1]{\ldb{#1}\rdb}       % item quoted by double brckets
\newcommand{\bdb}[1]{\bldb{#1}\brdb}    % item quoted by bold face
                                        % double breckets

% Usage: \balgo ... \ealgo
\newcommand{\balgo}{
   \begin{description}
   \parskip=0pt
   \topsep=0pt
}
\newcommand{\ealgo}{
   \end{description}
}

%\newcommand{\algorithm}[4]{
 %       \begin{scriptsize}
 %       \begin{tabbing}
  %              {\bf Procedure} #1 \\
  %      XXX\={\bf output:}X\= \+\kill
  %      {\bf input:}\>\+ #2\-\\
  %      {\bf output:}\>\+ #3\-\\[0.1in]
  %      XXX\=XXX\=XXX\=XXX\=XXX\=XXX\=\kill
  %      #4 \-\\
   %     {\bf end};
   %     \end{tabbing}
   %     \end{scriptsize}
%}
\newcommand{\while}[2]{
        {\bf while} (#1) {\bf do}\+\\
        #2\-\\
        {\bf end-while}
}
\newcommand{\for}[2]{
        {\bf for} (#1) {\bf do}\+\\
        #2\-\\
        {\bf end-for}
}
\newcommand{\ifthen}[2]{
        {\bf if} (#1) {\bf then}\+\\
        #2\-\\
        {\bf end-if}
}
%\newcommand{\ifthenelse}[3]{
 %       {\bf if} (#1) {\bf then}\+\\
  %      #2\-\\
   %     {\bf else}\+\\
    %    #3\-\\
     %   {\bf end-if}
%}
\newcommand{\rptuntil}[2]{
        {\bf repeat}\+\\
        #1\-\\
        {\bf until} (#2)
}
\newcommand{\return}[1]{{\bf return} #1}
\newcommand{\ass}{$\leftarrow$}

%
% Define algorithm commands
%
% Usage: the algorithm with only input, but no output,
%       \inalgorithm{<name>}{<input parameters>}{<the algorithms>}
%       \while{<condition>}{<while loop body>}
%       \for{<condition>}{<for loop body>}
%       \ifthen{<condition>}{<then part>}
%       \ifthenelse{<condition>}{<then part>}{<else part>}
%       \rptuntil{<loop body>}{<condition>}
%
\newcommand{\inalgorithm}[3]{
        \begin{small}
        \begin{tabbing}
                {\bf Procedure} #1 \\
        {\bf input:}X\=  \kill
        {\bf input:}\>\+ #2\-\\
        {\bf begin} \\
        XXX\=XXX\=XXX\=XXX\=XXX\=XXX\=\kill
        #3 \\
        {\bf end}.
        \end{tabbing}
        \end{small}
}

